An empirical study on declined proposals: why are these proposals declined?

Design-level decisions in open-source software (OSS) projects are often made through structured mechanisms such as proposals, which require substantial community discussion and review. Despite their importance, the proposal process is resource-intensive and often leads to contributor frustration, especially when proposals are declined without clear feedback. Yet, the reasons behind proposal rejection remain poorly understood, limiting opportunities to streamline the process or guide contributors effectively. This study investigates the characteristics and outcomes of proposals in the Go programming language to understand why proposals are declined and how such outcomes might be anticipated. We conduct a mixed-method empirical study on 1,091 proposals submitted to the Go project. We quantify proposal outcomes, build a taxonomy of decline reasons, and evaluate large language models (LLMs) for predicting these outcomes. We find that proposals are more often declined than accepted, and resolution typically takes over a month. Only 14.7% of declined proposals are ever resubmitted. Through qualitative coding, we identify nine key reasons for proposal decline, such as duplication, limited use cases, or violations of project principles. This taxonomy can help contributors address issues in advance, e.g., checking for existing alternatives can reduce redundancy. We also demonstrate that GPT-based models can predict decline decisions early in the discussion (F1 score = 0.71 with partial comments), offering a practical tool for prioritizing review effort. Our findings reveal inefficiencies in the proposal process and highlight actionable opportunities for improving both contributor experience and reviewer workload by enabling early triage and guiding contributors to strengthen their proposals using a structured understanding of past decline reasons.

==> Makefile <==
#!/usr/bin/make -f

CP=cp
RM=rm -f
TARG=main
#TARG=main_latexdiff

.PHONY: all clean

all:$(TARG).pdf

.SUFFIXES: .pdf .tex .aux .bbl

.tex.pdf:
	@\
	aux=$(<:%.tex=%.aux);\
	$(CP) $$aux $$aux-;\
	pdflatex $<;\
	echo ========;\
	diff -q $$aux $$aux- > /dev/null;\
	if [ $$? -eq 0 ]; then\
		echo No need for second compile.;\
	else\
		bibtex $$aux;\
		echo ========;\
		$(CP) $$aux $$aux-;\
		pdflatex $<;\
		echo ========;\
		diff -q $$aux $$aux- > /dev/null;\
		if [ $$? -eq 0 ]; then\
			echo No need for third compile.;\
		else\
			pdflatex $<;\
		fi;\
	fi;\
	$(RM) $$aux-
	$(RM) $(TARG).{aux,log,blg,cut,out,xcp,gz,xcp}

clean:
	$(RM) $(TARG).{pdf,aux,log,blg,cut,out,xcp,gz,xcp}


==> figures/background/status.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%%
%% ============================================================================
%% ============================================================================	

\begin{figure}[t]
  \centering
      \includegraphics[width=0.95\columnwidth]{figures/background/pstatus.pdf}
  \caption{Relationship between proposal statuses and issue comments}
  \label{fig:background:status}
\end{figure}

==> figures/discussion/prediction-performance-gpt4o.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% exp19/03_01_evaluation.ipynb 
%% exp19/figures/gpt4o-accuracy.pdf
%% ============================================================================
%% ============================================================================	

\begin{figure}[t]
  \centering
      \includegraphics[width=\columnwidth]{figures/discussion/pgpt4o-accuracy.pdf}
  \caption{Prediction performance for the declined reasons with GPT-4o}
  \label{fig:discussion:accuracy-gpt4o}
\end{figure}

==> figures/discussion/prediction-performance.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% exp18/03_01_evaluation.ipynb 
%% exp18/figures/accuracy.pdf
%% ============================================================================
%% ============================================================================	

\begin{figure}[t]
  \centering
      \includegraphics[width=\columnwidth]{figures/discussion/paccuracy.pdf}
  \caption{Prediction performance for the declined reasons with GPT-3.5-turbo}
  \label{fig:discussion:accuracy}
\end{figure}

==> figures/rq1/all_linked_issues.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% replication/rq1/05_make_barplot.ipynb
%% replication/rq1/plot/all_linked_issues.pdf
%% OLD
%% replication/rq1/04_make_barplot.R
%% replication/rq1/plot/all_linked_issues.pdf
%% ============================================================================
%% ============================================================================	

\begin{figure}[t]
  \centering
      \includegraphics[width=0.5\columnwidth]{figures/rq1/pall_linked_issues.pdf}
  \caption{Proportion of linked declined proposals}
  \label{fig:linked-declined-proposals}
\end{figure}

==> figures/rq1/num_issues_category.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% replication/rq1/05_make_barplot.ipynb
%% replication/rq1/plot/num_issues_category.pdf
%% OLD
%% replication/rq1/02_make_barplot.R
%% replication/rq1/plot/num_issues_category.pdf
%% ============================================================================
%% ============================================================================	


\begin{figure}[t]
  \centering
      \includegraphics[width=0.95\columnwidth]{figures/rq1/pnum_issues_category.pdf}
  \caption{Proportion of proposal states}
  \label{fig:proposal-statuses}
\end{figure}

==> figures/rq1/reappeared_issue_results.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% replication/rq1/04_make_barplot.R
%% replication/rq1/plot/reappeared_issue_results.pdf
%% ============================================================================
%% ============================================================================	


\begin{figure}[t]
  \centering
      \includegraphics[width=0.5\columnwidth]{figures/rq1/preappeared_issue_results.pdf}
  \caption{Proportion of accepted/declined reappeared proposals}
  \label{fig:reappeared-proposal-results}
\end{figure}

==> figures/rq2/change_type.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% exp23/02_compute.ipynb
%% exp23/plot/change_type_accept.pdf
%% exp23/plot/change_type_decline.pdf
%% ============================================================================
%% ============================================================================	

\begin{figure}[t]
  \centering
  \subfigure[Accepted proposals]{\includegraphics[width=\columnwidth]{./figures/rq2/pchange_type_accept.pdf}
  \label{fig:rq2:change-type-accept}}
  \subfigure[Declined proposals]{\includegraphics[width=\columnwidth]{./figures/rq2/pchange_type_decline.pdf}
  \label{fig:rq2:change-type-decline}}
  \caption{ 
    Proportion of prediction transition for accepted and declined proposals
  }
  \label{fig:rq2:change-type}
\end{figure}







==> figures/rq2/evaluation.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% exp17/05_01_makeplot.ipynb
%% exp17/plot/evaluation.pdf
%% OLD versions
%% exp17/03_01_makeplot.R (exp17/02_07_evaluation.ipynbでデータを作成する, Accuracy(Declined)は削除する)
%% exp17/plot/evaluation.pdf
%% OLD versions
%% exp9/02_03_makeplot.R (exp9/02_02_evaluation.ipynbでデータを作成する)
%% exp9/plot/evaluation.pdf
%% ============================================================================
%% ============================================================================	

\begin{figure}[t]
  \centering
      \includegraphics[width=\columnwidth]{figures/rq2/pevaluation.pdf}
  \caption{Prediction performance based on all comments (All) and no comments (NoComments) prior to the decision}
  \label{fig:rq2:evaluation}
\end{figure}

==> figures/rq2/rq2_overview.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% exp17/01_01_create_db.ipynb, 01_02, 02_02_prepare_data.py
%% ============================================================================
%% ============================================================================	

\begin{figure}[t]
  \centering
      \includegraphics[width=\columnwidth]{figures/rq2/prq2_overview.pdf}
  \caption{Data collection for RQ2}
  \label{fig:rq2:overview}
\end{figure}

==> figures/rq3/code-freq.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% exp15/02_for_sheet.ipynb 
%% exp15/01_count_codes.ipynb 
%% exp15/figures/freq.pdf
%% ============================================================================
%% ============================================================================	

\begin{figure}[h]
  \centering
      \includegraphics[width=\columnwidth]{figures/rq3/pfreq.pdf}
  \caption{Frequency of the discovered reasons for declined proposals}
  \label{fig:rq3:code-freq}
\end{figure}

==> sections/rq4.tex <==
\section{\RQfour{}}
%\section{Inferring Declined Reasons}
\label{sec:rq4}
%RQ4: \emph{\RQfour{}}
%\mahmoud{The section seems to have results. Hence, I think it should not be Discussion section, but rather a new RQ. The reason why I am suggesting this is that our analysis in RQ2 demonstrates the feasibility of anticipating declined proposals, while RQ3 establishes a taxonomy of the reasons for these decisions. Then, this section comes to provide an initial investigation into the capabilities of GPT-3.5-turbo for predicting reasons for declined proposals, in order to reduce the workload of open-source software (OSS) maintainers and contributors.}

%\masa{Need to discuss: Do we need to add examples? Not only the reasons in this RQ but also the taxonomy in RQ3. Check Mahmoud's comment: (check comment out here)}
%\mahmoud{For the reasons, can we come up with headings, e.g., a title for each reason. For example, I can see that the first reason is about: "Subjective nature of certain reasons". The second one could be "Need for complex inference", then for the last one could be: "Independence from Proposal Discussions". Also, I am not sure if we did it already, but it might be interesting to have an example for each reason in the Results section (not in this section), just for the reader to refer to what we say about the reasons in this section.}

%\subsection{Motivation}
%\mahmoud{If this section turns to be RQ, I'd suggest we split Approach and Motivation.}
Our findings from previous research questions highlight the complexity of understanding and anticipating declined proposals. RQ2 demonstrates that it is possible to predict whether a proposal will be declined, while RQ3 establishes a taxonomy of decline reasons, offering structured insights into why proposals are rejected. 
However, identifying why a proposal is likely to be declined remains a challenge for contributors, as it requires a deep understanding of Go’s design philosophy, ecosystem constraints, and community expectations.
Accurately predicting the reason for a declined proposal could provide early, actionable feedback to contributors, enabling them to revise their proposals before extensive discussions take place. This approach could also reduce the workload for maintainers by minimizing redundant discussions and clarifying potential issues upfront.
Therefore, this RQ conducts an initial investigation into the capabilities of GPT-3.5-turbo to predict the specific reasons for declined proposals. 
% RQ2 demonstrates that declined proposals can be anticipated, while RQ3 establishes a taxonomy of the reasons for declined proposals. In this study, we conducted an initial investigation into the capabilities of GPT-3.5-turbo to predict the reasons for declined proposals. As discussed in previous sections, such predictions could help reduce the workload of maintainers and contributors.

\subsection{Approach}
The prediction setting for this RQ aligns with the methodology established in RQ2.
We employ GPT-3.5-turbo to predict the reasons for declined proposals. The initial dataset consisted of 142 declined proposals. However, due to the input token limitations specific to GPT-3.5-turbo, two proposals were excluded, resulting in a final dataset of 140 proposals. 
For each proposal, we use all comments made prior to the likely accept/decline decision to ensure the predictions are based only on information available at the time of discussion.

To assess the upper-bound performance of the prediction task, we also employ GPT-4o--a more advanced language model capable of handling larger inputs.
We apply this model to the full set of 142 declined proposals, allowing for a comparative analysis of prediction capabilities between the two models.
% The prediction setting is consistent with RQ1. We employed GPT-3.5-turbo to predict the declined reasons for 142 proposals. However, due to the input token limitations specific to GPT-3.5-turbo, two proposals were excluded, resulting in a final dataset of 140 declined proposals. For each proposal, we utilized all comments made prior to the likely accept/decline decision.

% Additionally, to assess the current maximum prediction performance, we also employed GPT-4o to anticipate the declined reasons for the full set of 142 proposals.

%\input{./figures/discussion/prediction-performance.tex}
\input{./tables/discussion/prediction-performance-gpt35.tex}
\subsection{Results}

%%============New version
%========
%
%========
%========

We evaluate the ability of GPT-3.5-turbo and GPT-4o to predict the reasons for declined proposals. \tab{tab:discussion:accuracy} and \tab{tab:discussion:accuracy-gpt4o} present the performance of both models across the identified reasons.

\observation{Reasons grounded in existing data, such as Duplication and Existing Alternatives, are predicted with higher accuracy.} \label{ob:rq4:existing-data}
\tab{tab:discussion:accuracy} shows that the GPT-3.5-turbo model achieves its highest accuracy for Duplication (69.2\%) and Existing Alternatives (64.3\%). 
These reasons can often be inferred from explicit data sources, such as source code repositories, issue reports, and mailing lists, which the model may have been exposed to during training. 
This suggests that when the reasons are grounded in objective and verifiable information, the model is better equipped to make accurate predictions.

\observation{Reasons involving subjective judgment, complex inference, or independent decisions are more challenging to predict.} \label{ob:rq4:limit-gpt35}
For reasons such as Poor Feasibility, Limited Use Cases, No Consensus Reached, Breaking Go’s Principles, and Lack of Knowledge, GPT-3.5-turbo struggles, with accuracies falling below 40\%. 
The underlying challenges are threefold:
\begin{itemize}
    \item \textit{Subjective Judgments.} Reasons like Poor Feasibility, Limited Use Cases, and No Consensus Reached are subjective and depend on maintainers' personal judgment. For instance, what qualifies as a ``limited'' use case or a ``feasible'' solution can vary among reviewers. This variability makes it difficult for models to generalize effectively.

    \item \textit{Complex Inference.} Reasons such as Breaking Go’s Principles and Lack of Knowledge require deep contextual inference. While Go’s philosophy is documented, assessing whether a specific proposal violates these principles is non-trivial and often relies on nuanced understanding.

    \item \textit{Independent Decisions.}  Reasons such as Deprecated Proposals and License Problems often emerge independently of ongoing discussions. These decisions can be sudden and unrelated to the content of the proposal, making them particularly difficult for models to predict.
\end{itemize}

%\input{./figures/discussion/prediction-performance-gpt4o.tex}
\input{./tables/discussion/prediction-performance-gpt4o.tex}
\observation{GPT-4o substantially improves predictions for subjective reasons but struggles with complex inference and independent decisions.} \label{ob:rq4:limit-gpt4o}
\tab{tab:discussion:accuracy-gpt4o} shows that GPT-4o considerably enhances prediction accuracy for subjective reasons, such as Limited Use Cases (12.5\% → 68.8\%) and No Consensus Reached (33.3\% → 53.8\%). 
This suggests that advancements in GPT models can improve the handling of subjective judgments.
However, we can observe a decline in accuracy with GPT-4o for the Poor Feasibility reason, suggesting that model improvements can occasionally misinterpret edge cases. Furthermore, even with GPT-4o, performance for Breaking Go’s Principles and Lack of Knowledge remains low, indicating the inherent difficulty of reasoning about abstract or philosophical aspects.
Similarly, predictions for Deprecated Proposals and License Problems remained below 10\% for both models. 
As these reasons often arise unexpectedly, independent of prior discussion, the model lacks sufficient context to anticipate them. 
% These findings highlight the need for additional data sources beyond proposal discussions to improve prediction for such categories.


%%============Old version
%========
%
%========
%========
% \observation{GPT-3.5-turbo can accurately anticipate Duplication and Existing alternatives, achieving over 60\% accuracy.}
% \fig{fig:discussion:accuracy} shows the prediction performance for the declined reasons using GPT-3.5-turbo, with Duplication and Existing alternatives ranking as the top two reasons for which our prediction model, GPT-3.5-turbo, performs well, with accuracies of 69.2\% and 64.3\%, respectively.

% One possible reason for this performance is that these reasons can be inferred from existing data sources such as source code repositories, issues, and mailing lists. Since GPT-3.5-turbo may be trained on such existing data, we deduce that the model is well-suited for predicting these types of reasons.


% \observation{The prediction model does not perform well for other reasons, less than 40\%.}
% Specifically, except for Duplication and Existing alternatives, GPT-3.5-turbo fails to achieve high performance, with accuracies below 40\%.
% We deduce the following three reasons for this difference:
% \begin{itemize}
%   \item{\textbf{Subjective nature:}}
% The first reason for this difference is that some reasons are relatively subjective compared to Duplication and Existing alternatives: Poor feasibility, Limited use cases, and No consensus reached. For instance, Limited use cases refers to scenarios where the scope addressed by the proposal is restricted. In such cases, it is challenging to establish a clear definition of what ``limited'' actually means, as it relatively depends on the subjective judgment of OSS maintainers. As a result, GPT-3.5-turbo may struggle to perform well for these subjective reasons. 
%   \item{\textbf{Complex inference:}}
% The second reason is that some reasons require inference beyond the given information: Breaking Go's principles and Lack of knowledge. For example, Breaking Go’s principles refers to cases where a proposal violates Go’s philosophy. While Go’s philosophy is documented in text, it is necessary to infer whether a specific proposal might contradict these principles. Similarly, Lack of Knowledge requires inferring whether a proposal may violate certain underlying premises. In contrast, reasons like Existing alternatives can be identified by simply understanding the explicitly stated information, such as the official Go documentation. 
%   \item{\textbf{Independence from proposal discussions:}}
% The third reason is that the decisions of some reasons are often independent of the ongoing discussion and occur unexpectedly: Deprecated Proposals and License Problem. For instance, even if a proposal is actively being discussed, participants might suddenly identify another better proposal, leading to the current one being deprecated. This decision is independent of any prior discussions.
% Similarly, in the case of License Problem, a proposal may be declined suddenly if a contributor disagrees with the contribution terms, regardless of the previous discussion. 
% \end{itemize}

% \input{./figures/discussion/prediction-performance-gpt4o.tex}
% \observation{GPT-4o improves the performance of the model for reasons that are relatively subjective.}
% \fig{fig:discussion:accuracy-gpt4o} shows the prediction performance using GPT-4o, where significant improvements can be observed for Limited Use Cases (12.5\% to 68.8\%) and No Consensus Reached (33.3\% to 53.8\%).
% These reasons rely heavily on the subjective judgment of OSS maintainers. Thus, enhancing the GPT model in the future could further improve its ability to handle subjective judgments more accurately.

% Note that we deduce that Poor Feasibility is a relatively subjective reason. However, we observe a decrease in prediction performance when using GPT-4o. This suggests that, in some cases, enhancing the GPT model may inadvertently reduce accuracy for certain edge cases.

% \observation{Inferring whether a proposal may violate certain underlying philosophies and premises is challenging.}
% We observe that even with GPT-4o, the prediction performance for Breaking Go’s Principles and Lack of Knowledge remains low. This result suggests that researchers need to develop specific solutions to better support the prediction of declined reasons.

% \observation{Deprecated Proposals and License Problem are challenging reasons to predict.}
% The prediction performance for these categories is below 10\% for both GPT models. 
% As described above, this decision is independent of any prior discussions.
% To accurately anticipate these reasons, additional data sources beyond the proposal discussions are required.

% \input{tables/discussion/category.tex}

% \observation{The declined reasons can be classified into four categories based on the type of information required to anticipate them: \emph{existing data}, \emph{judgment by OSS maintainers}, \emph{inference}, and \emph{independent}.}
% This discussion suggests that the reasons classified under the categories of existing data and judgment by OSS maintainers can be anticipated with relatively high accuracy. However, the categories of inference and independent present greater challenges. Future studies are necessary to improve the prediction of declined reasons in these categories. \tab{tab:discussion:category} summarizes the categories and the corresponding reasons.

% - GPT4oでpoor feasibilityの結果が下がってしまう．なんで？
% - limited use caseとno consensus reachedの結果が上がる．これらはsubjectiveと言えそう
% - Breaking Gos principlesやlack of knowledgeの結果は低いまま．philosophyやpremiseは明確に記述されていないからか？

%\masa{Do we need to add something from our manual analysis?}
%\masa{RQ4? two GPT models converse each other and result in a good prediction for declined proposals? I'm quite interested in this point. Currently, we don't get good results when only using the title and description. However, when we use all comments, we get good results. This is because developers converse each other and provide context information to GPT models. Does GPT model's conversation with each other provide context information? Please check the comment}
%\masa{TODO Masa Please check my JP comment}
% この理由は予測モデルがGo開発のコンテキストを知らないことである．RQ2で示した通り，ソフトウェア開発においてはGo開発における一般常識やworkaroundなどさまざまな文章化されていない知識が存在する．コメントでの議論はこういった知識を補完する．そのため，GPTにはProposalのタイトルとdescriptionを見せられただけでは結論を出すには十分ではないことがわかる．
% どうして少ないコメントでは予測がうまくいかないのか？（RQ3）．その理由として，上で挙げているようにコンテキストの情報が不足しているというりゆうが考えられる．

% result
% - duplicationとexsiting alternativesでは高い精度が出た (既存のデータソースを利用しているから？)
% - 他の対象に対しての予測精度は低い（subjectiveであることは一つの要因．limited use caseなどは人間が読めば読み取れるが，絶対的な基準があるわけではなかった，例を示す）
% - deprecated proposalsは予測精度が非常に低かった (deprecatedとわかるのは議論の後に外部情報からなので，コメントのみでは予測が難しい)
% - GPT4でも予測精度は上がらないため，追加の情報が必要になる（RAG的な？fine tune？）


\summarybox{Key Insights of RQ4}
{
GPT-3.5-turbo performs best when predicting reasons grounded in explicit data, such as Duplication and Existing Alternatives (up to 69.2\% accuracy). However, it struggles with reasons involving subjective judgment (Limited Use Cases, No Consensus), complex inference (e.g., Breaking Go’s Principles), or independent decisions (e.g., Deprecated Proposals), with accuracies below 40\%. GPT-4o improves predictions for subjective reasons (e.g., Limited Use Cases rises from 12.5\% to 68.8\%) but still underperforms on inference-heavy and unpredictable cases, showing that certain decline reasons remain inherently hard to anticipate from discussion alone.
  % \textcolor{red}{Declined reasons can be predicted with a large language model.} However, reasons requiring complex inference (Breaking Go’s Principles, Lack of Knowledge) or arising from independent decisions (Deprecated Proposals, License Problems) remain challenging to predict\textcolor{red}{, even with a large language model. Future studies are necessary to predict declined reasons in these categories.}
  %The ability to predict declined reasons varies based on the type of information required. Reasons grounded in existing data (Duplication, Existing Alternatives) are predicted with high accuracy. In contrast, reasons involving subjective judgments (Limited Use Cases, No Consensus Reached) show moderate improvements with advanced models like GPT-4o. However, reasons requiring complex inference (Breaking Go’s Principles, Lack of Knowledge) or arising from independent decisions (Deprecated Proposals, License Problems) remain challenging to predict, even with more advanced models.
}
  % Our prediction model accurately anticipates the reasons in the existing data category, such as duplicates or existing alternatives, indicating its ability to effectively leverage patterns from existing data sources to make precise predictions. However, the model struggles with other categories. Specifically, three reasons are highly subjective (\eg, limited use cases), two require inference (\eg, lack of knowledge), and two are independent of any prior discussion (\eg, deprecated proposals). When utilizing the latest GPT model, prediction performance improves for the subjective category, while it remains unchanged for the inference and independent categories.
  % Our prediction model accurately anticipates the reasons for the existing data category: duplicates or existing alternatives, indicating its ability to effectively leverage patterns from existing data sources to make precise predictions.
  % However, the model does not perform well for other reasons. Three reasons are highly subjective (\eg, limited use cases), two reasons require inference (\eg, lack of knowledge), and the other two reasons are independent of any prior discussion (\eg, deprecated proposals).
  % When utilizing the latest GPT model, the prediction performance improves for the subjective category whereas the performance remains unchanged for the inference and independent categories. 
  %Even when utilizing the latest GPT model, the prediction performance does not show significant improvement. This suggests that the issue may lie not in the capability of the model, but in the inherent subjectivity of certain reasons, which makes it challenging to develop a prediction model for declined reasons that can effectively support maintainers and contributors.
  %, making it difficult to establish clear criteria for whether to accept or decline a proposal,

==> sections/versions/implication_ver1.tex <==
\section{Implication}
\label{sec:implication}

==> tables/discussion/category.tex <==

\begin{table}[t]
    \caption{Categories of declined reasons by information type required for anticipation}
\label{tab:discussion:category}
\begin{center}
\scalebox{1.0}{
    \begin{tabular}{ll}
    \toprule
		\multicolumn{1}{c}{\textbf{Category}} & \multicolumn{1}{c}{\textbf{Reason}}\\
    \midrule
    \multirow{2}{*}{Existing data} & Existing alternatives\\
                                   & Duplication\\
    \midrule
                                & Poor feasibility\\
    Judgment by OSS maintainers & Limited use cases\\
                                & No consensus reached\\
    \midrule
    \multirow{2}{*}{Inference}  & Breaking go’s principles\\
                                & Lack of knowledge \\
    \midrule
    \multirow{2}{*}{Independent} & License problem\\
                                 & Deprecated proposals\\
    \bottomrule
    \end{tabular}
    }
    \end{center}
\end{table}

% \emph{existing data}
% Deprecated proposals
% Existing alternatives
% Duplication
% 
% \emph{judgment by OSS maintainers}
% Poor feasibility
% Limited use cases
% No consensus reached
% 
% \emph{inference}
% Breaking go’s principles
% Lack of knowledge
% 
% \emph{others}
% License problem






==> tables/discussion/prediction-performance-gpt35.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% exp18/03_01_evaluation.ipynb 
%% exp18/results/gpt35_result_out.csv
%% ============================================================================
%% ============================================================================	

\begin{table}[t]
\caption{Prediction performance for the declined reasons with GPT-3.5-turbo}
\label{tab:discussion:accuracy}
\begin{center}
\scalebox{1.0}{
    \begin{tabular}{llr}
    \toprule
    \multicolumn{1}{c}{\textbf{Index}}&\multicolumn{1}{c}{\textbf{Category}}&\multicolumn{1}{c}{\textbf{Accuracy}}\\
    \midrule
    R7&Duplication&69.2\%(9/13)\\
    R5&Existing alternatives&64.3\%(9/14)\\
    R1&Poor feasibility&37.5\%(9/24)\\
    R8&No consensus reached&33.3\%(4/12)\\
    R4&Breaking Go's principles&15.0\%(3/20)\\
    R3&Limited use cases&12.5\%(2/16)\\
    R6&Lack of knowledge&7.7\%(1/13)\\
    R2&Deprecated proposals&3.7\%(1/27)\\
    R9&License problem&0.0\%(0/1)\\
    \bottomrule
    \end{tabular}
    }
    \end{center}
\end{table}



==> tables/discussion/prediction-performance-gpt4o.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% exp19/03_01_evaluation.ipynb 
%% exp19/results/gpt4o_result_out.csv
%% ============================================================================
%% ============================================================================	

\begin{table}[t]
\caption{Prediction performance for the declined reasons with GPT-4o}
\label{tab:discussion:accuracy-gpt4o}
\begin{center}
\scalebox{1.0}{
    \begin{tabular}{llrr}
    \toprule
    \multicolumn{1}{c}{\textbf{Index}}&\multicolumn{1}{c}{\textbf{Category}}&\multicolumn{1}{c}{\textbf{Accuracy}}&\multicolumn{1}{c}{\textbf{Diff}}\\
    \midrule
R7&Duplication&76.9\%(10/13)&$^{\textcolor{red}{+7.7}}$\\
R3&Limited use cases&68.8\%(11/16)&$^{\textcolor{red}{+56.3}}$\\
R5&Existing alternatives&64.3\%(9/14)&$^{\textcolor{red}{+0.0}}$\\
R8&No consensus reached&53.8\%(7/13)&$^{\textcolor{red}{+20.5}}$\\
R1&Poor feasibility&25.0\%(6/24)&$^{\textcolor{blue}{-12.5}}$\\
R4&Breaking Go's principles&25.0\%(5/20)&$^{\textcolor{red}{+10.0}}$\\
R6&Lack of knowledge&7.7\%(1/13)&$^{\textcolor{red}{+0.0}}$\\
R2&Deprecated proposals&7.1\%(2/28)&$^{\textcolor{red}{+3.4}}$\\
R9&License problem&0.0\%(0/1)&$^{\textcolor{red}{+0.0}}$\\
    \bottomrule
    \end{tabular}
    }
    \end{center}
\end{table}


%    Duplication&76.9\%(10/13)\\
%    Limited use cases&68.8\%(11/16)\\
%    Existing alternatives&64.3\%(9/14)\\
%    No consensus reached&53.8\%(7/13)\\
%    Poor feasibility&25.0\%(6/24)\\
%    Breaking Go's principles&25.0\%(5/20)\\
%    Lack of knowledge&7.7\%(1/13)\\
%    Deprecated proposals&7.1\%(2/28)\\
%    License problem&0.0\%(0/1)\\

==> tables/rq1/linked-proposals.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% 
%% ============================================================================
%% ============================================================================	


% \begin{table}[t]
\begin{table}[t]
    \caption{Numbers of linked new/declined proposals}
\label{tab:rq1:linked-proposals}
\begin{center}
\scalebox{1.0}{
    \begin{tabular}{cc}
    \toprule
		\multicolumn{1}{c}{Linked new proposals} & \multicolumn{1}{c}{Linked declined proposals}\\
    \midrule
    75&66\\
    \bottomrule
    \end{tabular}
    }
    \end{center}
\end{table}








==> tables/rq2/confusion_all.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% exp17/02_07_evaluation.ipynb
%% exp17/tables/confusion_matrix_all.csv
%% OLD versions
%% exp9/02_02_evaluation.ipynb
%% exp9/tables/confusion_matrix_all.csv
%% ============================================================================
%% ============================================================================	

\begin{table}[t]
\centering
\caption{Confusion matrix for accepted and declined proposals when using all comments}
\label{tab:rq2:confusion_all}
\begin{tabular}{ccc}
\toprule
& \textbf{Prediction Accepted} & \textbf{Prediction Declined} \\
\midrule
\textbf{Accepted} & 89&29\\
\textbf{Declined} & 9&133\\
\bottomrule
\end{tabular}
\end{table}



==> tables/rq2/confusion_nocomments.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% exp17/02_07_evaluation.ipynb
%% exp17/tables/confusion_matrix_nocomments.csv
%% OLD versions
%% exp9/02_02_evaluation.ipynb
%% exp9/tables/confusion_matrix_nocomments.csv
%% ============================================================================
%% ============================================================================	

\begin{table}[t]
\centering
\caption{Confusion matrix for accepted and declined proposals without using comments}
\label{tab:rq2:confusion_nocomments}
\begin{tabular}{ccc}
\toprule
& \textbf{Prediction Accepted} & \textbf{Prediction Declined} \\
\midrule
\textbf{Accepted} & 83&35\\
\textbf{Declined} & 53&89\\
\bottomrule
\end{tabular}
\end{table}



==> tables/rq2/likely-to-final.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% 
%% ============================================================================
%% ============================================================================	


\begin{table}[t]
    \caption{Proportion of proposals based on their likely and final decisions}
\label{tab:rq2:likely-to-final}
\begin{center}
\end{center}
\end{table}








==> tables/rq2/transition_patterns.tex <==
%% ============================================================================
%% PLEASE DON"T REMOVE THIS COMMENT
%% ============================================================================
%% ============================================================================
%% ============================================================================	

\begin{table}[t]
  \centering
  \caption{Prediction transition patterns}
  \label{tab:transition_patterns}
  \begin{tabular}{cl}
    \toprule
    \textbf{Pattern Code} & \multicolumn{1}{c}{\textbf{Description}} \\
    \midrule
    1 & All predictions are correct \\
    2 & All predictions are incorrect \\
    3 & Single transition: correct to incorrect \\
    4 & Single transition: incorrect to correct \\
    5 & Multiple transitions (starting with correct) \\
    6 & Multiple transitions (starting with incorrect) \\
    \bottomrule
    \end{tabular}
\end{table}

% , e.g., correct $\rightarrow$ incorrect $\rightarrow$ correct
%, e.g., incorrect $\rightarrow$ correct $\rightarrow$ incorrect






